Hiding Symbols and Functions: New Metrics and Constructions for Information-Theoretic Security

We present information-theoretic definitions and results for analyzing symmetric-key encryption schemes beyond the perfect secrecy regime, i.e. when perfect secrecy is not attained. We adopt two lines of analysis, one based on lossless source coding, and another akin to rate-distortion theory. We start by presenting a new information-theoretic metric for security, called symbol secrecy, and derive associated fundamental bounds. We then introduce list-source codes (LSCs), which are a general framework for mapping a key length (entropy) to a list size that an eavesdropper has to resolve in order to recover a secret message. We provide explicit constructions of LSCs, and demonstrate that, when the source is uniformly distributed, the highest level of symbol secrecy for a fixed key length can be achieved through a construction based on minimum-distance separable (MDS) codes. Using an analysis related to rate-distortion theory, we then show how symbol secrecy can be used to determine the probability that an eavesdropper correctly reconstructs functions of the original plaintext. We illustrate how these bounds can be applied to characterize security properties of symmetric-key encryption schemes, and, in particular, extend security claims based on symbol secrecy to a functional setting.

==> generalSource.tex <==

\section{List-source codes for general source models}
\label{sec:general}

The previous results hold for i.i.d. source models. However, for more general
sources the analysis becomes significantly more convoluted, since multiple
list-source encoded messages can reveal information about each other.
Considering that encryption is performed over multiple blocks of source symbols,
the list size will not necessarily grow if these block are correlated. %The
%following simple example describes how a linear list-source code can fail
%completely when applied directly to a Markovian source.

%\begin{example}
%Assume that $X$ is a Markovian source with two states, $S_0$ and $S_1$. We
%consider the outputs as elements of $\mathbb{F}_2$, and that no source coding is used. When in state $S_0$,
%the source outputs a sequence of $n$ 0's, and on the next transition goes to
%state $S_1$ w.p. 1/2 and stays in the same state w.p. 1/2. Analogously, when in
%state $S_1$, the source outputs a sequence of $n$ 1's, and transitions to $S_0$
%or stays in the same state with equal probability. Even though individually each
%bit produced by the source has probability 1/2 of being a 1 or a 0, if we encode
%a block of length $n$ of this source using a linear LSC (and assuming that the
%sequence of $n$ 0s and $n$ 1s belong to different cosets), an adversary can
%trivially resolve which was the original source sequence.
%\end{example}

In general, given an output $\bX=X_1,\dots,X_n$ of $n$ correlated source symbols, and
using scheme 1, what is observed by an
eavesdropper is the coset valued sequence of random elements
$\{H(s_n(\bX))\}$, $H$ being the parity check
matrix. Since $\bX$ is a correlated source of symbols, there is
no a priori reason to expect that the coset valued process will
not be correlated. For example if $\bX$ forms a Markov chain,
then the coset valued process is a function of a Markov chain; although it will not, in general, form a Markov chain itself, it
will still have correlations. These correlations could effectively
reduce the list size that an eavesdropper must search and, consequently, reduce the effectiveness of the scheme. Reducing or eliminating
correlations in the coset valued process would counteract the
impact of this vulnerability.


Different approaches can be taken to resolve this issue. In general, the key to
reducing the effect of the correlation between codewords is to encode larger
block lengths. More precisely, let $\bX_1,\bX_2,\dots, \bX_N$ be $N$ blocks of
symbols produced by a Markov source, such that $\bX_i \in \Xn$ and
$p(\bX_1,\dots,\bX_N)= p(\bX_1)p(\bX_2|\bX_1)\dots p(\bX_N|\bX_{N-1})$. Instead
of  encoding each block individually, the transmitter can compute
$\bY^{nNR}=f(\bX_1,\dots,\bX_N)$.

The previous approach has the disadvantage of requiring long block lengths and
possibly high implementation complexity. We note, however, that the encoding
procedure over multiple blocks does not necessarily have to be performed
independently. For example, one possible approach for overcoming edge-effect
correlations between codewords is to define
$\bY_1=f(\bX_1,\bX_2),\bY_2=f(\bX_2,\bX_3),\dots$, and so forth. This approach
reduces the edge effects of correlation between codewords, in particular when
the individual sequences $\bX_i$ are already significantly long. 


We note that, when probabilistic encryption \cite{katz_introduction_2007}  is required
over multiple blocks, the source encoded symbols in scheme 1 can be
combined with the output of a pseudorandom number generator (PRG) before being
multiplied by the parity check matrix. This would provide  the necessary randomization of the
output. The initial seed of the PRG can then be transmitted to the legitimate
receiver in phase II of scheme \ref{scheme:prac}. 




==> privacy.tex <==
\section{Connections to Privacy and Anonymity}

